Dysfluencies Seldom Come Alone -- Detection as a Multi-Label Problem

Specially adapted speech recognition models are necessary to handle stuttered speech. For these to be used in a targeted manner, stuttered speech must be reliably detected. Recent works have treated stuttering as a multi-class classification problem or viewed detecting each dysfluency type as an isolated task; that does not capture the nature of stuttering, where one dysfluency seldom comes alone, i.e., co-occurs with others. This work explores an approach based on a modified wav2vec 2.0 system for end-to-end stuttering detection and classification as a multi-label problem. The method is evaluated on combinations of three datasets containing English and German stuttered speech, yielding state-of-the-art results for stuttering detection on the SEP-28k-Extended dataset. Experimental results provide evidence for the transferability of features and the generalizability of the method across datasets and languages.

==> 03_data_pre_table.tex <==
% Only 64\% of Fbank are uniquely labeled
% SEP28k 70 \%
% KSoF 79\%
\subsection{SEP-28k and \fb}\label{ss:sep}
SEP-28k is a speech corpus containing stuttered speech extracted from podcasts \cite{lea_SEP28kDatasetStuttering_2021}. 
The 28177 clips where annotated by three naive annotators with five types dysfluency labels: blocks, prolongations, sound repetitions, word repetitions, and interjections.
The corpus also contains an additional 4144 clips that were extracted from the interview part of the the adults who stutter dataset of the \fb corpus \cite{bernsteinratner_FluencyBankNew_2018}, that were relabeled using the same protocol.

The SEP-28k corpus does not contain pre-defined data partitions or a suggested evaluation scheme.
Previous works failed to publish their splits and have reported to the use of non-speaker exclusive splits, which can yield to overoptimistic results \cite{bayerl_InfluenceDatasetPartitioning_2022}. 
We want to enable the comparability of methods and reproducibility of our research and therefore use the speaker-exclusive SEP28k-Extended data partitioning and the additional meta-data provided by \cite{bayerl_InfluenceDatasetPartitioning_2022}\footnote{Available: \protect\url{https://github.com/th-nuernberg/ml-stuttering-events-dataset-extended}}.
Gender and speaker information for the \fb corpus were taken taken from the metadata provided by the original authors of \fb \cite{bernsteinratner_FluencyBankNew_2018}. 
% There exists no pre-defined split for that dataset. 
We use a balanced split regarding gender and label distribution, consisting of six individuals ($\sim$800 clips), seven in the development set ($\sim$800 clips), and 19 in the training partition ($\sim$3300 clips), as used by \cite{bayerl_DetectingDysfluenciesStuttering_2022a}.\footnote{\protect \url{https://tinyurl.com/24vm6dec}}

\subsection{Kassel State of Fluency}
The Kassel State of Fluency (KSoF) dataset contains recordings from 37 PWS in German.
The dataset consists of 5597 3-sec long clips extracted from stuttering-therapy recordings.
The clips were labeled similarly to the SEP-28k dataset \cite{lea_SEP28kDatasetStuttering_2021} with the same five stuttering labels and a sixth label, speech modifications, which marks a clip as containing a person using speech technique known as fluency shaping, which is learned by PWs in stuttering therapy and is supposed to help them overcome their stuttering \cite{bayerl_KSoFKasselState_2022}.

The data and the labels are fully compatible with the datasets described in \cref{ss:sep}.
In our experiments, we utilize the gender-label for multi-task learning and use the train, development and test split of the dataset.

\subsection{Multi- and cross lingual training and inference}
\sep and \fb are almost balanced w.r.t. the labels of each core-symptom (between 8.1\% and 13.3\% of clips), interjections (21.2\%, 27.3\%), and no dysfluencies in 56.9\% and 54.1\% of cases. 
Whereas the \ksof~ dataset has few labeled word repetitions (3.8\%) and many blocks (20\%).
Compared to the other datasets fluent labels are underrepresented (24.75\%), as people int therapy try avoid stuttering by using modified speech (24.44\%) \cite{lea_SEP28kDatasetStuttering_2021,bayerl_KSoFKasselState_2022}. 

To evaluate cross-lingual and cross-dataset training performance, we define two combinations of datasets in addition to the \ksof, \fb, and \sepE splits. 
ENG is a combination of the \fb and \sepE and MIXED as a combination of \ksof, \fb, and \sepE. 
MIXED and \ksof are trained using seven classes (Modified, Blocks, Interjections, Prolongation, Sound Repetitions, Word Repetitions, No Dysfluencies), \fb, \sepE, and ENG are trained to detect six classes (Modified, Blocks, Interjections, Prolongation, Sound Repetitions, Word Repetitions).
